Splat-Nav: Safe Real-Time Robot Navigation in Gaussian Splatting Maps

We present Splat-Nav, a real-time robot navigation pipeline for Gaussian Splatting (GSplat) scenes, a powerful new 3D scene representation. Splat-Nav consists of two components: 1) Splat-Plan, a safe planning module, and 2) Splat-Loc, a robust vision-based pose estimation module. Splat-Plan builds a safe-by-construction polytope corridor through the map based on mathematically rigorous collision constraints and then constructs a B\'ezier curve trajectory through this corridor. Splat-Loc provides real-time recursive state estimates given only an RGB feed from an on-board camera, leveraging the point-cloud representation inherent in GSplat scenes. Working together, these modules give robots the ability to recursively re-plan smooth and safe trajectories to goal locations. Goals can be specified with position coordinates, or with language commands by using a semantic GSplat. We demonstrate improved safety compared to point cloud-based methods in extensive simulation experiments. In a total of 126 hardware flights, we demonstrate equivalent safety and speed compared to motion capture and visual odometry, but without a manual frame alignment required by those methods. We show online re-planning at more than 2 Hz and pose estimation at about 25 Hz, an order of magnitude faster than Neural Radiance Field (NeRF)-based navigation methods, thereby enabling real-time navigation. We provide experiment videos on our project page at https://chengine.github.io/splatnav/. Our codebase and ROS nodes can be found at https://github.com/chengine/splatnav.

==> sections/overview.tex <==
% \section{Splat-Nav Overview}
% \label{sec:overview}
% {
% \color{blue}

% Splat-Nav comprises a lightweight pose estimation module, Splat-Loc, coupled with a planning module, Splat-Plan, working interdependently to enable safe navigation from RGB-only (monocular) camera observations. We illustrate the architecture of Splat-Nav in \Cref{fig:splat_nav_architectire}.

% \begin{figure}[th]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/explainers/splat_nav_architecture.png}
%     \caption{(Temporary Illustration) Splat-Nav is composed of Splat-Loc, for real-time localization from monocular images, and Splat-Nav, for real-time trajectory planning within safe flight corridors
%     .}
%     \label{fig:splat_nav_architectire}
% \end{figure}

% Given an incoming RGB frame, Splat-Loc performs PnP-based localization, leveraging the GSplat map to estimate the RGB and depth values rendered at candidate poses, which is utilized to compute the extrinsic parameters of the drone's onboard camera and, ultimately, its pose. Splat-Plan takes in the estimated pose computed by Splat-Loc to generate an initial trajectory, which is subsequently optimized to lie within safe flight corridors, constructed from the geometric and spatial attributes of the GSplat Map. Moreover, the pose estimation module Splat-Loc utilizes the safe flight corridors computed by Splat-Plan to project the drone's estimated pose into a safe area of the environment.
% In the subsequent sections, we elaborate on Splat-Loc and Splat-Plan. \textcolor{red}{Mac: there is no need for a full section for this.  It would be best to combine it with another section or remove it.  Also figure 4 is redundant to Fig. 2.  It's literally the textbook architecture for robot navigation.  Readers will get annoyed if we spend time on this.  If this is in response to R1.1, I wouldn't do that.  R1.1 was bizarre and I think we can simply point to the revised intro and other revisions as evidence that we addressed that concern.}


% }
